Prevention of Microarchitectural Covert Channels on an Open-Source 64-bit RISC-V Core

Covert channels enable information leakage across security boundaries of the operating system. Microarchitectural covert channels exploit changes in execution timing resulting from competing access to limited hardware resources. We use the recent experimental support for time protection, aimed at preventing covert channels, in the seL4 microkernel and evaluate the efficacy of the mechanisms against five known channels on Ariane, an open-source 64-bit application-class RISC-V core. We confirm that without hardware support, these defences are expensive and incomplete. We show that the addition of a single-instruction extension to the RISC-V ISA, that flushes microarchitectural state, can enable the OS to close all five evaluated covert channels with low increase in context switch costs and negligible hardware overhead. We conclude that such a mechanism is essential for security.

==> Makefile <==
# Generic paper Makefile
#
# For usage hints, "make help"
#
#  To create a LaTeX diff against the hg "tip" revision, use the target
#  "diff" (or "viewdiff").
#  To use a revision other than "tip", speciff DIFF=x on the 
#  make command line to choose the revision x.
#  WILL NOT WORK, ASSUMES USING hg
#

# Verbosity
ifeq (${V},1)
Q:=
else
Q:=@
endif

.PHONY: all

BIBDIR     ?= 
LaTeXEnv   = 
BibTexEnv  = 
BibFiles   = defs,extra,combined,systems,fm,other

LaTeX      = ${LaTeXEnv} pdflatex -interaction=nonstopmode
# Uncomment the following for "unsw" when using TrueType fonts (which they require)
#LaTeX      = ${LaTeXEnv} lualatex -interaction=nonstopmode
AcmSty	   = ACM-Reference-Format.bst acmart.cls
LaTeXdiff  = ./tools/latexdiff
BibTeX     = ${BibTexEnv} bibtex
BibExport  = ./tools/bibexport.sh
Fig2Eps    = fig2dev -L eps
Dia2Eps    = dia -t eps -e
AS         = $(shell which as)
CC         = $(shell which gcc)
GnuPlot	   = gnuplot
Inkscape   = $(shell which inkscape)
Eps2Pdf	   = epstopdf --outfile
PdfView	   = xpdf
Pdf2Ps	   = pdf2ps
Md2Pdf	   = pandoc
RmCR       = tr -d '\r'
sed        = $(shell which sed)
Lpr 	   = lpr
mv	   = mv
awk	   = awk
R	   = R
ToGray	   = convert -colorspace gray
Git	   = git

# Use either "report" or "paper", depending on the template.
# To add a further target, simply append the basename of the .tex file here
# NOTE: for the "simple", "report" and "unsw" templates, uncomment the lualatex line above!
TexFiles = $(wildcard content/*.tex)
Targets    = carrv20-covert-channels


# CONFIGURATION OPTIONS
# =====================

# Extra figures that aren't supplied as dia, gnuplot or fig sources
# (eg figures already supplied in PDF, or supplied in EPS).
# List with pdf extensions.
# Note that PDF files should be added to the repo with an additional -shipped extension,
# but should appear here with just the .pdf extension.
ExtraFigs= # should list all non-generated figure files


# Any other stuff that may be needed

# END CONFIGURATION OPTIONS
# =========================

Optional = $(addsuffix -diff, $(Targets))
All = $(Targets) $(Optional)
Diffopts= #--type=BWUNDERLINE #-c .latexdiffconfig --append-safecmd="Comment"

Perf_Sources = $(wildcard figures/*.perf)
Dia_Sources = $(wildcard figures/*.dia)
Fig_Sources = $(wildcard figures/*.fig)
Gnuplot_Sources = $(wildcard figures/*.gnuplot)
SVG_Sources = $(wildcard figures/*.svg)
R_Sources = $(wildcard figures/*.r)
Styles = $(wildcard *.sty)  $(wildcard *.cls)
Figures = $(Perf_Sources:.perf=.pdf) $(Dia_Sources:.dia=.pdf) $(Fig_Sources:.fig=.pdf) $(SVG_Sources:.svg=.pdf) $(Gnuplot_Sources:.gnuplot=.pdf)  $(R_Sources:.r=.pdf) $(ExtraFigs) 
GreyFigs = $(subst .pdf,-gr.pdf,$(subst figures/,./,$(wildcard figures/*.pdf)))

Pdf = $(addsuffix .pdf, $(Targets))
Bib = sources.bib
Tex = $(addsuffix .tex, $(Targets)) $(wildcard content/*.tex)
Diff_Pdf = $(addsuffix .pdf, $(Optional))

.PHONY: FORCE

all: pdf
diff: diff_pdf
FORCE: pdf
ps: $(Ps)
pdf: $(Figures) Makefile $(Pdf)
diff_pdf: $(Figures) Makefile $(Diff_Pdf)
grey:	$(GreyFigs)
gray:	grey

%-gr.pdf:	figures/%.pdf
	${ToGray} $< $@

%.pdf: %.perf ./tools/bargraph.pl
	@echo $< '->' $@
	${Q} ${BarGraph} -pdf $< > $@

%.pdf: %.eps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

%.pdf: %.ps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

%.eps: %.svg
	@echo $< '->' $@
	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
	${Q} ${Inkscape} -f $< -D -z -E $@ > /dev/null 2>&1

%.pdf: %.svg
	@echo $< '->' $@
	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
	${Q} ${Inkscape} -f $< -D -z -A $@ > /dev/null 2>&1

# This target allows you to add figures which have the extension .c_pp that
# correspond to .c sources. Your .c sources can use the lines '/*<*/' and
# '/*>*/' to surround parts of the source you don't want shown in your PDF.
# This allows you to write a .c file that can be compile-checked here and then
# remove extraneous lines for display.
%.c_pp: %.c
	@echo $< '->' $@
	${Q}$(if ${CC},${CC} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.s_pp: %.s
	@echo $< '->' $@
	${Q}$(if ${AS},${AS} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.eps: %.dia
	@echo $< '->' $@
	${Q} ${Dia2Eps} $@ $<

%.eps: %.fig
	@echo $< '->' $@
	${Q} ${Fig2Eps} $< $@

%.eps: %.gnuplot
	@echo $< '->' $@
	${Q} ${GnuPlot} $<

%.eps: %.r
	@echo $< '->' $@
	${Q} ${R} --vanilla < $<

%.pdf: %.pdf-shipped
	cp $< $@

%.pdf:	%.md
	$(Md2Pdf) $< -o $@

%.view:	%.pdf
	$(PdfView) $<

view: pdf
	${Q}for i in $(Pdf); do \
		$(PdfView) $$i & \
	done

viewdiff: diff
	${Q}for i in $(Diff_Pdf); do \
		$(PdfView) $$i & \
	done

print: pdf
	${Q}for i in $(Pdf); do \
		$(Lpr) $$i \
	done

clean:
	rm -f *.aux *.toc *.bbl *.blg *.dvi *.log *.pstex* *.eps *.cb *.brf \
		*.rel *.idx *.out *.ps *-diff.* *.mps .log *.diff *.cut tmp.* $(GreyFigs)

realclean: clean
	rm -f *~ *.pdf *.tgz

tar:	realclean
	( p=`pwd` && d=`basename "$$p"` && cd .. && \
	  tar cfz $$d.tgz $$d && \
	  mv $$d.tgz $$d )

help:
	@echo "Main targets: all diff camera view viewdiff print clean realclean tar"
	@echo "'make diff' will show changes to head revision"
	@echo "'make grey' will generate greyscale figures (for B&W readibility check)"
	@echo "'make DIFF=<rev> diff' will show changes to revision <rev>"
	@echo 'Avoid TeX \def with arguments, this breaks latexdiff (use \newcommand)'

##############################################################################

DIFF ?= tip

%-diff.dvi: %-diff.tex

%-diff.tex: %.tex FORCE
	@echo "version for mercurial, will not work with git!"
	@false
	@echo "====> Retrieving revision $(DIFF) of $<"
	hg cat -r $(DIFF) $<  > $(@:-diff.tex=-$(DIFF)-diff.tex)
	@echo "====> Creating diff of revision $(DIFF) of $<"
	$(LaTeXdiff) $(Diffopts) $(@:-diff.tex=-$(DIFF)-diff.tex) $< | \
	${RmCR} > $@

.PHONY: FORCE
FORCE:

# don't delete %.aux intermediates
.SECONDARY:

##############################################################################

Rerun = '(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)'
Rerun_Bib = 'No file.*\.bbl|Citation.*undefined'
Undefined = '((Reference|Citation).*undefined)|(Label.*multiply defined)'
Error = '^! '
BibWarn = '^Warning--'
LaTeXWarn = ' [Ww]arning: '

%.pdf: %.tex $(TexFiles) $(Bib) $(Figures) $(Styles) Makefile
	${Q}if test $*.bbl -ot $(Bib); then rm -f $*.bbl; fi
	@echo "====> LaTeX first pass: $(<)"
	${Q}$(LaTeX) $< >.log || if egrep -q $(Error) $*.log ; then cat .log; rm $@; false ; fi
	${Q}if egrep -q $(Rerun_Bib) $*.log ; then echo "====> BibTex" && ( $(BibTeX) $* > .log || ( cat .log ; false ) ) && echo "====> LaTeX BibTeX pass" && $(LaTeX) >.log $< || if egrep -q $(Error) $*.log ; then cat .log; rm $@; false ; fi ; fi
	${Q}if egrep -q $(Rerun) $*.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) $*.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) $*.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	@echo "====> Undefined references and citations in $(<):"
	@egrep -i $(Undefined) $*.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" $*.log || echo "None."
	@echo "====> Warnings:"
	${Q}bibw=`if test -e $*.blg; then grep -c $(BibWarn) $*.blg; else echo 0; fi`; \
	texw=`grep -c $(LaTeXWarn) $*.log`; \
	if [ "$$bibw" -gt 0 ]; then echo " $$bibw BibTeX\c"; fi; \
	if [ "$$texw" -gt 0 ]; then echo " $$texw LaTeX\c"; fi; \
	if [ "$$bibw$$texw" = 00 ]; then echo "None."; \
	else echo ". 'make warn' will show them."; fi

warn:
	@echo "====> BibTeX warnings from" *.blg
	@grep $(BibWarn) *.blg || echo "None."
	@echo "====> LaTeX warnings from" *.log
	@grep $(LaTeXWarn) *.log || echo "None."

##############################################################################
# Generate a list of FIXMEs 
fixmes: 
	${Q}for i in $(Tex); do \
		echo "FIXMEs in $$i:"; \
		nl -b a $$i | grep "FIXME{" | nl -b a; \
		echo -n "Total FIXMES: " && grep "FIXME{" $$i | wc -l; \
		echo; \
	done


==> content/08_discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     <file_name>.tex                                             %
%%%%%                                                                 %
%%%%% Author:      <author>                                           %
%%%%% Created:     <date>                                             %
%%%%% Description: <description>                                      %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Discussion}

\subsection{Hardware-Software Contract}

\subsubsection{Flush Instruction}

\subsubsection{Hardware Parameters}
e.g. cache size, worst case flush latency


\subsection{Future Work}
